In-Context Explainers: Harnessing LLMs for Explaining Black Box Models

Recent advancements in Large Language Models (LLMs) have demonstrated exceptional capabilities in complex tasks like machine translation, commonsense reasoning, and language understanding. One of the primary reasons for the adaptability of LLMs in such diverse tasks is their in-context learning (ICL) capability, which allows them to perform well on new tasks by simply using a few task samples in the prompt. Despite their effectiveness in enhancing the performance of LLMs on diverse language and tabular tasks, these methods have not been thoroughly explored for their potential to generate post hoc explanations. In this work, we carry out one of the first explorations to analyze the effectiveness of LLMs in explaining other complex predictive models using ICL. To this end, we propose a novel framework, In-Context Explainers, comprising of three novel approaches that exploit the ICL capabilities of LLMs to explain the predictions made by other predictive models. We conduct extensive analysis with these approaches on real-world tabular and text datasets and demonstrate that LLMs are capable of explaining other predictive models similar to state-of-the-art post hoc explainers, opening up promising avenues for future research into LLM-based post hoc explanations of complex predictive models.

==> 010newintro.tex <==
\section{Introduction}
\label{sec:intro}

\looseness=-1 Over the past decade, machine learning (ML) models have become ubiquitous across various industries and applications. With their increasing use in critical applications (\eg healthcare, financial systems, and crime forecasting), it becomes essential to ensure that ML developers and practitioners understand and trust their decisions. To this end, several approaches~\cite{ribeiro2016should,ribeiro2018anchors,smilkov2017smoothgrad,sundararajan2017axiomatic,lundberg2017unified,shrikumar2017learning} have been proposed in explainable artificial intelligence (XAI) literature to generate explanations for understanding model predictions. However, these explanation methods are highly sensitive to changes in their hyperparameters~\cite{yeh2019fidelity,bansal2020sam}, require access to the underlying black box ML model~\cite{lundberg2017unified, ribeiro2016should}, and/or are often computationally expensive~\cite{situ2021learning}, thus impeding reproducibility and the trust of relevant stakeholders.

Recent advancements in machine learning (ML) research have been significantly influenced by generative models, especially Large Language Models (LLMs) as highlighted by ~\cite{radford17:learning}.
These models have demonstrated exceptional capabilities, outperforming previous state-of-the-art models in complex tasks like machine learning translation~\cite{hendy2023good}, language understanding~\cite{brown2020language}, commonsense reasoning~\cite{wei2022chain,krishna2023post}, and coding tasks~\cite{bubeck2023sparks}. However, there is very little work on systematically analyzing the reliability of LLMs as explanation methods. While recent research has used LLMs to explain what patterns in a piece of text cause a neuron to activate, they simply explain correlations between the network input and specific neurons and do not explain what causes model behavior at a mechanistic level~\cite{bills2023language}. 
Thus, the potential of LLMs to serve as reliable explainers and enhance the understanding of ML models has not been sufficiently explored. 
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{ICML/results/LLM_framework.pdf}
    \vskip -0.1in
    \caption{\small
        \looseness=-1
        \xhdr{Overview of LLM explanation generation process} Given a dataset and model to explain, we provide 1) different prompting strategies to generate explanations using LLMs, 2) functions to parse LLM-based explanations, 3) utility functions to support new LLMs, and 4) diverse performance metrics to evaluate the faithfulness of explanations.
    }
    \vspace{-0.15in}
    \label{fig:framework}
\end{figure*}

\looseness=-1\xhdr{Present work} In this work, we investigate a relatively unexplored question: ``\textit{Can LLMs explain the behavior of other complex predictive models?}'' (see Fig.~\ref{fig:framework}). To answer this question, we exploit the in-context learning (ICL)~\cite{liu2023pre} capabilities of LLMs which enable these models to learn from a small set of of examples provided at inference time~\cite{akyurek2022learning}. We propose two broad ICL-based prompting strategies, namely perturbation-based and explanation-based ICL, which provide the foundation for exploring the explanation-generating capabilities of state-of-the-art LLMs. Perturbation-based ICL builds on the ideas from explainable AI literature which involve constructing local linear approximations\hbox{~\cite{ribeiro2016should}} to explain the predictions made by a given ML model. To this end, we provide instance perturbations and their corresponding model outputs in the prompt to the LLM and ask the LLM to explain (i.e., output the top features driving) these predictions. We consider a couple of variants under this strategy, namely, \vanillaExp (\pc) and \instructionICL (\pcg). For \pc, we prompt the LLM to use its chain-of-thought reasoning by starting with ``Think about the question." For \pcg, we add detailed guidelines in the prompt for generating explanations. In our \iclExp strategy, we prompt the LLM with a small, random selection of model input-output pairs and their explanations (created using a state-of-the-art post hoc explanation method) to generate explanations for new samples.

\looseness=-1 We analyze the effectiveness of LLMs in explaining other predictive models on four real-world datasets, two black box models, and three \textsc{Gpt} models. Our extensive investigation reveals the following key findings: \circled{\textbf{1}} LLMs can generate faithful explanations that are on par with gradient-based methods (despite these methods having access to the underlying black box model); \circled{\textbf{2}} LLMs can mimic the behavior of six state-of-the-art explanation methods using the proposed \iclExp prompting strategy; \circled{\textbf{3}} On average across four datasets, we find that providing the LLM with detailed guidelines showed more consistent and higher faithfulness scores than just providing generic instructions; \circled{\textbf{4}} We show the progressive improvement in the faithfulness of LLM-generated explanations with the advent of more advanced LLMs. Finally, our exploration highlights LLMs' effectiveness as post hoc explainers, paving the way for future research on LLM-generated explanations.
